The Physics Potential of SuperB

SuperB is a major new European e+e- collider facility to be built in Italy that will provide a precise study of the structure of New Physics beyond the Standard Model at energy scales above the LHC as well as a comprehensive program of Standard Model physics. In this article, I review the physics opportunities, the status of the accelerator and detector studies, and the future plans.

==> abstract.tex <==
SuperB is a major new European $e^+e^-$ collider facility to be built
  in Italy that will provide a precise study of the structure of New
  Physics beyond the Standard Model at energy scales above the LHC as
  well as a comprehensive program of Standard Model physics. In this
  article, I review the physics opportunities, the status of the
  accelerator and detector studies, and the future plans.

